Get More with LESS: Synthesizing Recurrence with KV Cache Compression for Efficient LLM Inference

Many computational factors limit broader deployment of large language models. In this paper, we focus on a memory bottleneck imposed by the key-value (KV) cache, a computational shortcut that requires storing previous KV pairs during decoding. While existing KV cache methods approach this problem by pruning or evicting large swaths of relatively less important KV pairs to dramatically reduce the memory footprint of the cache, they can have limited success in tasks that require recollecting a majority of previous tokens. To alleviate this issue, we propose LESS, a simple integration of a (nearly free) constant sized cache with eviction-based cache methods, such that all tokens can be queried at later decoding steps. Its ability to retain information throughout time shows merit on a variety of tasks where we demonstrate LESS can help reduce the performance gap from caching everything, sometimes even matching it, all while being efficient. Relevant code can be found at https://github.com/hdong920/LESS.

==> formulation.tex <==

\subsection{Problem formulation}
\label{sec:formulation}


% tensor mathematical model, assumption, goal
 
Suppose that the ground truth tensor $\bcX_\star \in \RR^{n_1 \times n_2 \times n_3}$ with multilinear rank $\br = (r_1, r_2, r_3)$ admits the following Tucker decomposition
\begin{equation} \label{tucker_star}
    \bcX_\star = \big( \bU_\star^{(1)}, \bU_\star^{(2)}, \bU_\star^{(3)} \big) \bcdot \bcG_\star,
\end{equation}
where $\bU^{(1)}_{\star}\in\RR^{n_1\times r_1}$, $\bU^{(2)}_{\star}\in\RR^{n_2\times r_2}$, $\bU^{(3)}_{\star}\in\RR^{n_3\times r_3}$ are the factor matrices along each mode,  and $\bcG_{\star}\in\RR^{r_1\times r_2\times r_3}$ is the core tensor. The Tucker decomposition is not unique since for any $\bQ^{(k)} \in \text{GL}(r_k)$, $k=1,2,3$, in view of \eqref{eq:multilinear}, we have
\begin{align*}
    \big(\bU^{(1)}, \bU^{(2)}, \bU^{(3)} \big) \bcdot \bcG = \big(\bU^{(1)} \bQ^{(1)}, \bU^{(2)} \bQ^{(2)}, \bU^{(3)} \bQ^{(3)} \big) \bcdot \bcG_{\bQ}
\end{align*}
where $\bcG_{\bQ} = \big((\bQ^{(1)})^{-1}, (\bQ^{(2)})^{-1}, (\bQ^{(3)})^{-1} \big) \bcdot \bcG$. Without loss of generality, to address ambiguity, we set the ground truth $\bF_{\star}=(\bU_{\star}^{(1)},\bU_{\star}^{(2)},\bU_{\star}^{(3)},\bcG_{\star})$ to satisfy that for each mode, $\bU_{\star}^{(k)} \in \RR^{n_k \times r_k}$ to have orthonormal columns, and 
\begin{equation} \label{eq:singular_value_matrix}
\Matricize{k}{\bcG_{\star}} \Matricize{k}{\bcG_{\star}}^\top = \big(\bSigma_{\star}^{(k)} \big)^2,
\end{equation} 
the squared singular value matrix $\bSigma_{\star}^{(k)}$ of $\Matricize{k}{\bcX_{\star}}$. This can be easily met, for example, by taking the tensor factors $\bF_{\star}$ as the HOSVD of $\bcX_{\star}$. 



\paragraph{Observation model and goal.} Suppose that we collect a set of corrupted observations of $\bcX_{\star}$ as
\begin{equation}\label{eq:obs_model}
\bcY = \bcX_{\star} + \bcS_{\star},
\end{equation}
where $\bcS_{\star}$ is the corruption tensor. The problem of tensor RPCA seeks to separate $\bcX_{\star}$ and $\bcS_{\star}$ from their sum $\bcY$ as efficiently and accurately as possible. %\edits{Note that when there are no corruptions, taking the HOSVD of $\bcY$ will return \eqref{tucker_star}, the desired Tucker decomposition of $\bcX_\star$.}
 
\paragraph{Key quantities.} Obviously, the tensor RPCA problem is ill-posed without imposing additional constraints on the low-rank tensor $\bcX_{\star}$ and the corruption tensor $\bcS_{\star}$, which are crucial in determining the performance of the proposed algorithm. We first introduce the incoherence parameter of the tensor $\bcX_\star $.  

  
\begin{definition}[Incoherence]
The incoherence parameter $\mu$ of $\bcX_\star $ is defined as
\begin{align}
     \mu := \max_k \left\{\frac{n_k}{r_k} \norm{\bU_\star^{(k)}}_{2, \infty}^2 \right\},
\end{align}
where $\bcX_\star = \big(\bU_\star^{(1)}, \bU_\star^{(2)}, \bU_\star^{(3)}\big) \bcdot \bcG_\star$ is its Tucker decomposition.
\end{definition}

The incoherence parameter roughly measures how spread the energy of $\bcX_\star$ is over its entries---the energy is more spread as $\mu$ gets smaller. Moreover, we define a new notion of condition number that measures the conditioning of the ground truth tensor $\bcX_\star$ as follows, which is weaker than previously used notions. 

\begin{definition}[Condition number]
The condition number $\kappa$ of $\bcX_{\star}$ is defined as
\begin{equation} \label{eq:reduced_kappa}
	\kappa  := \frac{\min_k \sigma_{\max}(\Matricize{k}{\bcX_\star})}{\min_k \sigma_{\min}(\Matricize{k}{\bcX_\star})}.
\end{equation}
\end{definition}
\noindent 
With slight abuse of terminology, denote 
\begin{align} \label{eq:sigma_min_X}
\sigma_{\min}(\bcX_{\star}) = \min_{k} \sigma_{\min}(\cM_k(\bcX_\star))
\end{align} 
as the minimum nonzero singular value of $\bcX_\star$.


\begin{remark} The above-defined condition number can be much smaller than the {\em worst-case} condition number $\kappa_s$ used in prior analyses \cite{tong2021scaling,cai2021generalized,han2020optimal}, which is defined as
\begin{equation} \label{eq:compare_kappa}
	\kappa_s := \frac{\max_k \sigma_{\max}(\Matricize{k}{\bcX_\star})}{\min_k \sigma_{\min}(\Matricize{k}{\bcX_\star})} \geq\frac{\min_k \sigma_{\max}(\Matricize{k}{\bcX_\star})}{\min_k \sigma_{\min}(\Matricize{k}{\bcX_\star})} =  \kappa.
\end{equation}
Furthermore, the condition number $\kappa$ is also upper bounded by the largest condition number of the matricization along different modes, i.e., $\kappa \leq \max_k \kappa_k  =\max_k  \frac{\sigma_{\max}(\Matricize{k}{\bcX_\star})}{\sigma_{\min}(\Matricize{k}{\bcX_\star})}  $.  
\end{remark}



Turning to the corruption tensor, we consider a deterministic sparsity model following the matrix case~\cite{chandrasekaran2011siam,netrapalli2014non,yi2016fast}, where $\bcS_{\star}$ contains at most a small fraction of nonzero entries per fiber. This is captured in the following definition. 

%\begin{definition}[$\alpha$-fraction sparsity]
%The corruption tensor $\bcS_{\star}$ is $\alpha$-fraction sparse, i.e., $\bcS_{\star}\in\bcS_{\alpha}$, where  
%\begin{multline}
%\bcS_{\alpha}\coloneqq \Big\{\bcS\in\RR^{n_{1}\times n_{2}\times n_3}:\; \|\bcS_{i_1,:,:}\|_{0}\le\alpha n_{2} n_{3}, \; \|\bcS_{:,i_2,:}\|_{0}\le\alpha n_{1} n_{3}, \; \|\bcS_{:,:,i_3}\|_{0}\le\alpha n_{1}n_{2},  \\
%  \mbox{ for all  } 1\leq i_k \leq n_k, \quad k=1,2,3 \Big\}.\label{eq:S_alpha}
%\end{multline}
%\end{definition}

\begin{definition}[$\alpha$-fraction sparsity]
The corruption tensor $\bcS_{\star}$ is $\alpha$-fraction sparse, i.e., $\bcS_{\star}\in\bcS_{\alpha}$, where  
\begin{multline}
\bcS_{\alpha}\coloneqq \Big\{\bcS\in\RR^{n_{1}\times n_{2}\times n_3}:\; \|\bcS_{i_1,i_2,:}\|_{0}\le\alpha n_{3}, \; \|\bcS_{i_1,:,i_3}\|_{0}\le\alpha n_{2}, \; \|\bcS_{:,i_2,i_3}\|_{0}\le\alpha n_{1},  \\
  \mbox{ for all  } 1\leq i_k \leq n_k, \quad k=1,2,3 \Big\}.\label{eq:S_alpha}
\end{multline}
\end{definition}
% consider mentioning some applications



%\edits{Equivalently, each row of $\Matricize{k}{\bcS_\star}$ contains at most $\alpha$-fraction nonzero entries for $k=1, 2, 3$.} 
With this setup in hand, we are now ready to describe the proposed algorithm.



==> result.tex <==
% !TEX root = ./Tensor_RPCA.tex

\section{Main results}

\input{formulation.tex}



\subsection{Proposed algorithm}


Our algorithm alternates between corruption removal and factor refinements. To remove the corruption, we use the following soft-shrinkage operator that trims the magnitudes of the entries by the amount of some carefully pre-set threshold.

\begin{definition}[Soft-shrinkage operator]
For an order-$3$ tensor $\bcX$, the soft-shrinkage operator $\Shrink{\zeta}{\cdot}:\, \mathbb{R}^{n_1\times n_2\times n_3} \mapsto \mathbb{R}^{n_1\times n_2\times n_3}$ with threshold $\zeta>0$ is defined as
\begin{align*}
    \big[\Shrink{\zeta}{\bcX}\big]_{i_1, i_2, i_3} := \sgn\big([\bcX]_{i_1, i_2, i_3}\big) \,\cdot\,\max\big(0, \big| [\bcX]_{i_1, i_2, i_3} \big| - \zeta \big) .
\end{align*}
\end{definition}
The soft-shrinkage operator $\Shrink{\zeta}{}$ sets entries with magnitudes smaller than $\zeta$ to $0$, while uniformly shrinking the magnitudes of the other entries by $\zeta$. At the beginning of each iteration, the corruption tensor is updated via
\begin{subequations} \label{eq:alg1_updates}
\begin{align} \label{eq:update_corruption} 
\bcS_{t+1}  = \Shrink{\zeta_{t+1}}{\bcY - \big(\bU_t^{(1)}, \bU_t^{(2)}, \bU_t^{(3)} \big) \bcdot \bcG_t},   
\end{align}
with the schedule $\zeta_t$ to be specified shortly. With the newly updated estimate of the corruption tensor, the tensor factors are then updated by scaled gradient descent \cite{tong2021scaling}, for which they they are computed according to \eqref{eq:ScaledGD} with respect to $\cL(\bF_t, \bcS_{t+1})$ in \eqref{eq:loss}:
\begin{align}
    \bU^{(k)}_{t+1} &= \bU^{(k)}_t - \eta \nabla_{\bU^{(k)}_t} \cL(\bF_t, \bcS_{t+1}) \big(\Breve{\bU}_t^{(k)\top} \Breve{\bU}_t^{(k)} \big)^{-1} \nonumber \\
%    &= \bU^{(k)}_t - \eta \left( \bU_t^{(k)} \Breve{\bU}_t^{(k)\top}   + \Matricize{k}{\bcS_{t+1}} -  \Matricize{k}{\bcY}\right) \Breve{\bU}_t^{(k)} \big(\Breve{\bU}_t^{(k)\top} \Breve{\bU}_t^{(k)} \big)^{-1} \nonumber \\
    &= (1 - \eta) \bU_t^{(k)} - \eta \big(\Matricize{k}{\bcS_{t+1}} -  \Matricize{k}{\bcY} \big)\Breve{\bU}_t^{(k)} \big(\Breve{\bU}_t^{(k)\top} \Breve{\bU}_t^{(k)} \big)^{-1} \label{a_update3}
    \end{align}
for $k=1,2,3$ and
\begin{align}    
    \bcG_{t+1} &= \bcG_t - \eta \left( \big( \bU^{(1)\top}_t \bU_t^{(1)} \big)^{-1}, \big(\bU^{(2)\top}_t \bU_t^{(2)} \big)^{-1}, \big(\bU^{(3)\top}_t \bU_t^{(3)}\big)^{-1} \right) \bcdot \nabla_{\bcG_t} \cL(\bF_t , \bcS_{t+1}) \nonumber \\
%    &= \bcG_t - \eta \left( \big(\bU^{(1)\top}_t \bU_t^{(1)}\big)^{-1} \bU_t^{(1)\top}, \big(\bU^{(2)\top}_t \bU_t^{(2)}\big)^{-1} \bU_t^{(2)\top}, \big(\bU^{(3)\top}_t \bU_t^{(3)}\big)^{-1} \bU_t^{(3)\top} \right)  \nonumber \\
%    & \qquad \qquad\qquad \bcdot \left( \big(\bU_t^{(1)}, \bU_t^{(2)}, \bU_t^{(3)} \big) \bcdot \bcG_t + \bcS_{t+1} - \bcY \right) \nonumber\\
    &= (1-\eta) \bcG_t - \eta\left( \big(\bU^{(1)\top}_t \bU_t^{(1)}\big)^{-1} \bU_t^{(1)\top}, \big(\bU^{(2)\top}_t \bU_t^{(2)}\big)^{-1} \bU_t^{(2)\top}, \big(\bU^{(3)\top}_t \bU_t^{(3)}\big)^{-1} \bU_t^{(3)\top} \right)  \bcdot \left(\bcS_{t+1} - \bcY \right). \label{g_update3}
\end{align}
\end{subequations}
Here, $\eta >0$ is the learning rate, and
\begin{equation*}
\Breve{\bU}_t^{(1)}:= \big(\bU_t^{(3)} \otimes \bU_t^{(2)} \big) \Matricize{1}{\bcG_t}^{\top}, \quad \Breve{\bU}_t^{(2)}:= \big(\bU_t^{(3)} \otimes \bU_t^{(1)} \big) \Matricize{2}{\bcG_t}^{\top},\; \mbox{and} \quad \Breve{\bU}_t^{(3)}:= \big(\bU_t^{(2)} \otimes \bU_t^{(1)} \big) \Matricize{3}{\bcG_t}^{\top}.
\end{equation*}

To complete the algorithm description, we still need to specify how to initialize the algorithm. We will estimate the tensor factors via the spectral method, by computing the HOSVD of the observation after applying the soft-shrinkage operator:
$$ \big (\bU_0^{(1)}, \bU_0^{(2)}, \bU_0^{(3)}, \bcG_0 \big) = \hosvd{\br}{\bcY -\bcS_0}, \qquad \mbox{where} \quad \bcS_0 =  \Shrink{\zeta_0}{\bcY}. $$
Altogether, we arrive at Algorithm \ref{alg:tensor_RPCA}, which we still dub as ScaledGD for simplicity. 


 
\begin{algorithm}[t]
\caption{ScaledGD for tensor robust principal component analysis}\label{alg:tensor_RPCA} 
\begin{algorithmic} 
\STATE \textbf{Input:} the observed tensor $\bcY$, the multilinear rank $\br$, learning rate $\eta$, and threshold schedule $\{\zeta_t\}_{t=0}^{T}$. 
\STATE \textbf{Initialization:} $\bcS_0 = \Shrink{\zeta_0}{\bcY}$ and $\big (\bU_0^{(1)}, \bU_0^{(2)}, \bU_0^{(3)}, \bcG_0 \big) = \hosvd{\br}{\bcY -\bcS_0}$.
\FOR{$t = 0, 1, \dots, T-1$}
    \STATE Update the corruption tensor $\bcS_{t+1}$ via \eqref{eq:update_corruption};
%    $$\bcS_{t+1} = \Shrink{\zeta_{t+1}}{\bcY - \big(\bU_t^{(1)}, \bU_t^{(2)}, \bU_t^{(3)} \big) \bcdot \bcG_t};$$
    \STATE Update the tensor factors $\bF_{t+1} = \big( \bU^{(1)}_{t+1},  \bU^{(2)}_{t+1},  \bU^{(3)}_{t+1},  \bcG_{t+1} \big)$ via \eqref{a_update3} and \eqref{g_update3};
    %\FOR{$k= 1, 2, 3$}
        % \State $\Breve{\bU}_t^{(k)} \gets (\bU^{(N)}_t \otimes \dots \otimes \bU^{(k+1)}_t \otimes \bU^{(k - 1)}_t \otimes \dots \otimes \bU^{(1)}_t) \Matricize{k}{\bcG_t}^\top$
%        \begin{align*} 
%         \bU^{(k)}_{t+1} & = (1 - \eta) \bU_t^{(k)} - \eta \Matricize{k}{\bcS_{t+1} - \bcY}\Breve{\bU}_t^{(k)} \big( \Breve{\bU}_t^{(k)\top} \Breve{\bU}_t^{(k)} \big)^{-1}, \qquad k=1,2,3;\\
%  %  \ENDFOR
%      \bcG_{t+1}  & = (1-\eta) \bcG_t - \eta \left( \big( \bU^{(1)\top}_t \bU_t^{(1)} \big)^{-1} \bU_t^{(1)\top}, \big( \bU^{(2)\top}_t \bU_t^{(2)} \big)^{-1} \bU_t^{(2)\top}, \big( \bU^{(3)\top}_t \bU_t^{(3)} \big)^{-1} \bU_t^{(3)\top}\right) \bcdot \left(\bcS_{t+1} - \bcY \right).
%      \end{align*}
%      where $\Breve{\bU}_t^{(1)}:= \big(\bU_t^{(3)} \otimes \bU_t^{(2)} \big) \Matricize{1}{\bcG_t}^{\top}$, $\Breve{\bU}_t^{(2)}:= \big(\bU_t^{(3)} \otimes \bU_t^{(1)} \big) \Matricize{2}{\bcG_t}^{\top}$, and $\Breve{\bU}_t^{(3)}:= \big(\bU_t^{(2)} \otimes \bU_t^{(1)} \big) \Matricize{3}{\bcG_t}^{\top}$.
\ENDFOR
\STATE \textbf{Output:} the tensor factors $ \bF_T = \big (\bU_{T}^{(1)}, \bU_T^{(2)}, \bU_T^{(3)}, \bcG_T \big) $.
\end{algorithmic} 
\end{algorithm}

%Un-matricizing (folding) the gradient, we will get $\nabla_{\bcG_t} \cL(\bF_t)$.
%\begin{align*}
%    \nabla_{\bcG_t} \cL(\bF_t) &= ((\bU_t^{(1)})^\top \bU_t^{(1)}, (\bU_t^{(2)})^\top \bU_t^{(2)}, (\bU_t^{(3)})^\top \bU_t^{(3)}) \bcdot \bcG_t + ((\bU_t^{(1)})^\top, (\bU_t^{(2)})^\top, (\bU_t^{(3)})^\top) \bcdot (\bcS_{t+1} - \bcY) \\
%    &= ((\bU_t^{(1)})^\top, (\bU_t^{(2)})^\top, (\bU_t^{(3)})^\top) \bcdot \left( ( \bU_t^{(1)}, \bU_t^{(2)}, \bU_t^{(3)}) \bcdot \bcG_t +  (\bcS_{t+1} - \bcY) \right)
%\end{align*}

%\begin{align*}
%    \nabla_{\bU_t^{(k)}} \cL(\bF_t) &= \frac{1}{2} \nabla_{\bU_t^{(k)}} \norm{\Matricize{k}{(\bU_t^{(1)}, \bU_t^{(2)}, \bU_t^{(3)}) \bcdot \bcG_t + \bcS_{t+1} - \bcY}}_{\fro}^2 \\
%    % &= \frac{1}{2} \nabla_{\bU_t^{(k)}} \norm{\bU_t^{(k)} \Matricize{k}{\bcG_t}(\bU_t^{(N)} \otimes \dots \otimes \bU_t^{(k+1)} \otimes \bU_t^{(k-1)} \otimes \dots \otimes \bU_t^{(1)})^\top + \Matricize{k}{\bcS_{t+1}} -  \Matricize{k}{\bcY}}_{\fro}^2 \\
%    &= \frac{1}{2} \nabla_{\bU_t^{(k)}} \norm{\bU_t^{(k)} (\Breve{\bU}_t^{(k)})^\top + \Matricize{k}{\bcS_{t+1}} -  \Matricize{k}{\bcY}}_{\fro}^2 \\
%    &= \frac{1}{2} \nabla_{\bU_t^{(k)}} \norm{\Breve{\bU}_t^{(k)} (\bU_t^{(k)})^\top  + \Matricize{k}{\bcS_{t+1}}^\top -  \Matricize{k}{\bcY}^\top}_{\fro}^2 \\
%    &= \left[(\Breve{\bU}_t^{(k)})^\top \left( \Breve{\bU}_t^{(k)} (\bU_t^{(k)})^\top  + \Matricize{k}{\bcS_{t+1}}^\top -  \Matricize{k}{\bcY}^\top\right)\right]^\top \\
%    &= \left( \bU_t^{(k)} (\Breve{\bU}_t^{(k)})^\top   + \Matricize{k}{\bcS_{t+1}} -  \Matricize{k}{\bcY}\right) \Breve{\bU}_t^{(k)}
%\end{align*}


\paragraph{Computational benefits.} It is worth highlighting that the proposed tensor RPCA algorithm possesses several computational benefits which might be of interest in applications.
\begin{itemize}

\item {\em Advantages over matrix RPCA algorithms.} While it is possible to matricize the input tensor and then apply the matrix RPCA algorithms, they can only exploit the low-rank structure along the mode that the tensor is unfolded, rather than along multiple rows simultaneously as in the tensor RPCA algorithm. In addition, the space complexity of storing and computing the factors is much higher for the matrix RPCA algorithms, where the size of the factors become multiplicative in terms of the tensor dimensions due to unfolding, rather than linear as in the tensor RPCA algorithm.
\item {\em Generalization to $N$-th order tensors.} Although the description of Algorithm \ref{alg:tensor_RPCA} is tailored to an order-$3$ tensor, our algorithm is easily generalizable to any $N$-th order tensor; in fact, Algorithm~\ref{alg:tensor_RPCA} can be applied almost verbatim by redefining
$$\Breve{\bU}_t^{(k)} = \big(\bU_t^{(N)} \otimes \cdots \otimes \bU_t^{(k+1)} \otimes \bU_t^{(k-1)} \otimes \cdots \otimes \bU_t^{(1)} \big) \Matricize{k}{\bcG_t}^\top, \qquad k=1,\ldots, N $$
to its natural high-order counterpart. This extension is numerically evaluated in our experiments in Section~\ref{sec:numerical}.

\item {\em Parallelizability.} At each iteration of the proposed algorithm, each tensor factor is updated independently as done in \eqref{a_update3} and \eqref{g_update3}, therefore we can update them in a parallel manner. This improvement becomes more apparent as the order of the tensor increases. %While the left and right matrix in the matrix algorithm can be parallelized, matricization of the input matrix will result in the update of the right matrix having enormous matrix operations.

    \item \textit{Selective modes to update}: If we know the underlying ground truth tensor is only low-rank along certain mode, we can choose to skip the iterative updates of the rest of the modes after initialization to reduce computational costs, which we demonstrate empirically in Section \ref{background_subtraction}. %While the theorems presented do not apply to this refinement, this works empirically, as demonstrated in Section \ref{background_subtraction}.
    
\end{itemize}

\begin{comment}
\paragraph{Benefits}
 
\begin{itemize}
    \item \textit{Preservation of Ranks}: To apply the matrix RPCA algorithm, we would need to matricize the input tensor. However, the rank of the resulting matrix would be dependent on the mode of matricization. As an extreme example, if we matricized along the third mode of a rank $(2, r, n)$ tensor, the matricized form would be of rank $n$, effectively destroying the low rank structure of the tensor. As another extreme example, if we matricize along the first mode and apply the matrix RPCA algorithm, we are ignoring the low rank structure of the second mode which leads to the next benefit.
    \item \textit{Simultaneous Compression}: The matrix RPCA algorithm assumes low rank of the matrix it is trying to retrieve, ignoring the low rank structure of the rest of the entire tensor. For instance, in a video background-foreground separation problem, it is common to matricize along the axis corresponding to the frames since the relatively unchanging background is what is assumed to be low rank. If the background itself is low rank, this will be ignored. The tensor RPCA algorithm can simultaneously extract the static background and the low rank representation of the background. 
    \item \textit{Selective Modes to Update}: If we know that the the rank of the a tensor is $(r, n, n)$, we can choose to skip the iterative updates of the last three modes after initialization to reduce computational costs. While the theorems presented do not apply to this refinement, this works empirically, as demonstrated in Section \ref{background_subtraction}.
    \item \textit{Parallelizability}: At each iteration of the algorithm, each factor is updated independently of each other, given last iteration's outputs and the sparse matrix of the current iteration. Therefore, we can update all these in parallel, and this improvement becomes more apparent as the order of the tensor increases. While the left and right matrix in the matrix algorithm can be parallelized, matricization of the input matrix will result in the update of the right matrix having enormous matrix operations.
    \item \textit{Space Complexity}: To store the vectors and singular values of the SVD of a rank $(r, r, r)$ tensor, we need to store $r(n + n^2 + 1)$ or $\mathcal{O}(n^2 r)$ numbers. To store the vectors and singular values of the Tucker decomposition, we need to store $r(3n + r^2)$ or $\mathcal{O}(3nr + r^3)$. Since $r << n$, we see that the Tucker decomposition is more space efficient.
\end{itemize}

\end{comment}


\subsection{Performance guarantees}

 
Motivated by the analysis in \cite{tong2021scaling}, we consider the following distance metric, which not only resolves the ambiguity in the Tucker decomposition, but also takes the preconditioning factor into consideration. 
\begin{definition}[Distance metric]
Letting $\bF := \big(\bU^{(1)}, \bU^{(2)}, \bU^{(3)}, \bcG \big)$ and $\bF_\star := \big(\bU_\star^{(1)}, \bU_\star^{(2)}, \bU_\star^{(3)}, \bcG_\star \big)$, denote
\begin{equation}\label{dist}
    \dist^2(\bF, \bF_\star) := \inf_{\bQ^{(k)} \in \GL(r_k)} \sum_{k=1}^{3} \norm{ \big(\bU^{(k)} \bQ^{(k)} - \bU^{(k)}_\star \big) \bSigma_\star^{(k)}}_{\fro}^2 + \norm{\big( (\bQ^{(1)})^{-1}, (\bQ^{(2)})^{-1}, (\bQ^{(3)})^{-1} \big) \bcdot \bcG- \bcG_\star}_{\fro}^2,
\end{equation}
where we recall $\bSigma_\star^{(k)}$ is the singular value matrix of $\Matricize{k}{\bcX_{\star}}$, $k=1,2,3$. Moreover, if the infimum is attained at the arguments $\{\bQ^{(k)}\}_{k=1}^3$, they are called the optimal alignment matrices between $\bF$ and $\bF_{\star}$.  
\end{definition}

%If $\dist(\bF, \bF_\star) < \sigma_{\min}(\bcX_\star)$, then the infimum is attained \cite[Lemma 6]{tong2021scaling}.

Fortunately, the proposed ScaledGD algorithm (cf.~Algorithm \ref{alg:tensor_RPCA}) provably recovers the ground truth tensor---as long as the fraction of corruptions is not too large---with proper choices of the tuning parameters, as captured in following theorem.
\begin{theorem} \label{main}
Let $\bcY = \bcX_\star + \bcS_\star \in \RR^{n_1 \times n_2 \times n_3}$, where $\bcX_\star$ is $\mu$-incoherent with multilinear rank $\br = (r_1, r_2, r_3)$, and $\bcS_\star$ is $\alpha$-sparse. Suppose that the threshold values $\{\zeta_k\}_{k=0}^\infty$ obey that $  \norm{\bcX_\star}_\infty \leq \zeta_0  \leq 2     \norm{\bcX_\star}_\infty$ and  $\zeta_{t+1} = \rho \zeta_{t}$, $t\geq 1$, for some properly tuned $\zeta_1: =  8 \sqrt{\frac{\mu^3 r_1 r_2 r_3}{n_1 n_2 n_3}}   \sigma_{\min}(\bcX_\star)
$ and $\frac{1}{7} \leq \eta \leq \frac{1}{4}$, where $\rho = 1-0.45\eta$. Then,  the iterates $\bcX_t =  \big(\bU_t^{(1)}, \bU_t^{(2)}, \bU_t^{(3)} \big) \bcdot \bcG_t$ satisfy
\begin{subequations} \label{eq:thm_claims}
\begin{align}
    \norm{ \bcX_t - \bcX_\star}_{\fro} &\leq 0.03 \rho^t  \sigma_{\min}(\bcX_\star) , \label{eq:fro_contraction}  \\ 
 \norm{ \bcX_t - \bcX_\star}_{\infty}  & \leq 8 \rho^t \sqrt{\frac{\mu^3 r_1 r_2 r_3}{n_1 n_2 n_3}}   \sigma_{\min}(\bcX_\star), \label{eq:entry_contraction} \\
 \norm{ \bcS_t - \bcS_\star}_{\infty}  & \leq 16 \rho^{t-1} \sqrt{\frac{\mu^3 r_1 r_2 r_3}{n_1 n_2 n_3}}   \sigma_{\min}(\bcX_\star) \label{eq:sparse_contraction}
\end{align}
\end{subequations}
for all $t\geq 0$, as long as  the level of corruptions obeys
 $\alpha \leq \frac{c_0}{\mu^2 r_1 r_2 r_3 \kappa}$
 for some sufficiently small $c_0>0$.
\end{theorem}

The value of $\rho$ was selected to simplify the proof and should not be taken as an optimal convergence rate.
In a nutshell, Theorem \ref{main} has the following immediate consequences: 
\begin{itemize}
\item \textbf{Exact recovery.} Upon appropriate choices of the parameters, if the level of corruptions $\alpha$ is small enough, i.e. not exceeding the order of $\frac{1}{\mu^2 r_1 r_2 r_3 \kappa}$, we can ensure that the proposed Algorithm \ref{alg:tensor_RPCA} exactly recovers the ground truth tensor $\bcX_\star$ even when the gross corruptions are arbitrary and adversarial. As mentioned earlier, our result significantly enlarges the range of allowable corruption levels for exact recovery when the outliers are evenly distributed across the fibers, compared with the prior art established in \cite{cai2021generalized}. 

\item \textbf{Constant linear rate of convergence.} The proposed ScaledGD algorithm (cf.~Algorithm \ref{alg:tensor_RPCA}) finds the ground truth tensor at a {\em constant} linear rate, which is independent of the condition number, from a carefully designed spectral initialization. Consequently, the proposed ScaledGD algorithm inherits the computational robustness against ill-conditioning as \cite{tong2021scaling}, even in the presence of gross outliers, as long as the thresholding operations are properly carried out.


\item \textbf{Refined entrywise error guarantees.} Furthermore, when $\mu=O(1)$ and $r =O(1)$, the entrywise error bound \eqref{eq:entry_contraction}---which is smaller than the Frobenius error \eqref{eq:fro_contraction} by a factor of $\sqrt{\frac{1}{n_1n_2n_3}}$---suggests the errors are distributed in an evenly manner across the entries for incoherent and low-rank tensors. The same applies to the entrywise error bound of the sparse tensor \eqref{eq:sparse_contraction} which exhibits similar behavior as \eqref{eq:entry_contraction}. To the best of our knowledge, this is the first time such a refined entrywise error analysis is established for tensor RPCA.
\end{itemize}



 
%the upper bound on distance to the ground truth and the data matrix error linearly converge to $0$ for appropriate choices of the step size $\eta$ and thresholding parameters, $\zeta_0$ and $\zeta_1$.This is similar to the matrix RPCA guarantee in \cite[Theorem 1]{cai2021learned}, which shows the existence of hyperparameters $\{\zeta_k\}_{k=0}^\infty$ such that recovery is guaranteed. In contrast, Theorem \ref{main} essentially guarantees recovery with just appropriately tuned $\zeta_0$ and $\zeta_1$.
%Later in this paper, we will show that if we choose our $\zeta_0$ and $\zeta_1$ carefully, we do not need to tune $\{\zeta_t\}_{t=2}^\infty$.

 
 


 
% 
%\begin{remark}
%\yc{to be merged as a comparison/discussion about algorithm design.}
% \cite{cai2021learned} also presents a variant of deep unfolding methods to tune the thresholding parameters $\zeta_t$ and step sizes for every iteration.
%However, while they guarantee convergence for a specific choice of $\{\zeta_t\}_{k=0}^\infty$, this choice is not implementable since this choice depends on knowledge of the distance between our estimated data matrix and the ground truth.
%For our tensor RPCA algorithm, we will make linear convergence more implementable by not only showing a range of values $\{\zeta_t\}_{k=0}^\infty$ can take and still guarantee linear convergence, but also demonstrating that one can just tune $\zeta_0$ and $\zeta_1$ instead of an infinite number of parameters for this guarantee to hold.
%\end{remark}

